Real-Time Verification for Distributed Cyber-Physical Systems

Safety-critical distributed cyber-physical systems (CPSs) have been found in a wide range of applications. Notably, they have displayed a great deal of utility in intelligent transportation, where autonomous vehicles communicate and cooperate with each other via a high-speed communication network. Such systems require an ability to identify maneuvers in real-time that cause dangerous circumstances and ensure the implementation always meets safety-critical requirements. In this paper, we propose a real-time decentralized reachability approach for safety verification of a distributed multi-agent CPS with the underlying assumption that all agents are time-synchronized with a low degree of error. In the proposed approach, each agent periodically computes its local reachable set and exchanges this reachable set with the other agents with the goal of verifying the system safety. Our method, implemented in Java, takes advantages of the timing information and the reachable set information that are available in the exchanged messages to reason about the safety of the whole system in a decentralized manner. Any particular agent can also perform local safety verification tasks based on their local clocks by analyzing the messages it receives. We applied the proposed method to verify, in real-time, the safety properties of a group of quadcopters performing a distributed search mission.

==> caseStudy.tex <==
\section{Case study}
\seclabel{caseStudy}
%

\dung{Tran and Luan will work on this section}

\dung{Motion dynamic of drone, cite from Nathan thesis, Luan will help with this}

\dung{Run realtime-reachability algorithm for each agent, Tran and Luan will work on this}

\dung{Run the real-time trace analysis, Tran, Luan and Prof. Taylor will work on this}

\subsection{Quadcopter dynamics}

%\begin{figure}[t]
	%\centering
		%\includegraphics[width=0.45\textwidth]{images/drone.pdf}
		%\caption{Body frame of a quadcopter.}
	%\figlabel{fig:drone}
%\end{figure}


We apply our framework for a distributed multi-agent systems where the agents are quadcopters. The dynamics of a quadcopter is given by the equations for acceleration in an three-dimensions coordination $(x,y,z)$ as follows~\cite{luukkonen2011modelling}.  
%
\begin{equation}\eqlabel{droneDynamics}
\begin{split}
&\ddot{x} = (\frac{f}{m})(\sin(\psi)\sin(\phi) + \cos(\psi)\sin(\theta)\cos(\phi)),\\
&\ddot{y} = (\frac{f}{m})(\sin(\psi)\sin(\theta)\cos(\phi) - \sin(\phi)\cos(\theta)),\\
&\ddot{z} = (\frac{f}{m})\cos(\theta)\cos(\phi) - g,
\end{split}
\end{equation}
%  
where $\theta$, $\phi$, and $\psi$ are the pitch, roll, and yaw angles in the body frame, $f = \sum_{i=1}^4T_i$ is sum of the propeller forces, $m$ is the mass of the quad-copter, and $g = 9.81 m/s^2$ is the gravitational acceleration constant. 

If the height of the quadcopter is remained constant and only planar motion to waypoints in the $(x,y)$ plane is desired, we can assume that $\ddot{z} = 0$, i,e., there is no acceleration in the vertical direction. This assumption yields:
%
\begin{equation*}
f = \frac{mg}{\cos(\theta)\cos(\phi)}.
\end{equation*}
% 

The quadcopter dynamics can be further simplified by assuming the quadcopter's planar orientation $\psi$ is zero. This assumption is reasonable in practice since the quadcopter's planar orientation $\psi$ can be measured and controlled to stay within a range $[-\epsilon, +\epsilon]$, where $\epsilon$ is a very small value. Substituting the above equation and $\psi = 0$ into~\eqref{droneDynamics}, we get the simplified model of the quadcopter as follows. 
%
\begin{equation}
\begin{split}
\ddot{x} = g*\tan(\theta), \\
\ddot{y} = g*\frac{\tan(\phi)}{\cos(\theta)}.
\end{split}
\end{equation}
%

To control the position of the quadcopter in the $(x,y)$ plane, two PID controllers are designed to supply the control inputs (i.e., the pitch $\theta$ and the roll $\phi$) for the quadcopter.   

\subsection{Experimental Evaluation}

% overview
%\sayan{Sridhar: Few sentences about implementation.}
In this section, we describe the platform used for developing distributed hybrid systems and the type of applications used to evaluate our approach for verification of global predicates. We also demonstrate the sensitivity of the algorithm with respect to the different parameters computed both statically and dynamically. Further, we demonstrate the applicability of the algorithm by presenting a deadlock detection example.

\subsection{Distributed Applications on \starl Android Platform}
% setup
%% STAR: overview of actual setup
All the traces used in experimental evaluation of our technique are generated from distributed programs written for Android devices~\cite{AndroidProg} controlling mobile robots. In our laboratory, we have implemented a Java-based framework, called \starl~\cite{ZimMit:2012}, on top of the Android operating system. \starl has implementations of 
\begin{inparaenum}[(a)]
\item unicast and multicast protocols, 
\item a library of high-level functions for accomplishing common distributed tasks (for example, mutual exclusion, leader election, synchronization, etc.), 
\item functions for accessing hardware sensors on the Android device (such as GPS sensors, accelerometers, and cameras), and 
\item motion-control functions (used in applications where each Android device is paired via Bluetooth with a mobile robot, such as an iRobot Create). 
\end{inparaenum}
For the purposes of the experiments in this paper, \starl provides a convenient abstraction for programming a swarm of mobile robots with many sensors, in Java, and over a standard operating system. Over the past year, we have used \starl to implement several applications such as peer-to-peer chat, geocasting, coordinated distributed search, flocking, and distributed traffic control~\cite{ZimMit:2012}. In almost all cases, our initial implementations violated some of the expected safety and progress properties of the application. Often the violations were not reproducible, which made it difficult and time consuming to find their root cause. This experience, at least in part, motivated the work reported in this paper.

In this paper, we use traces generated from three \starl applications: 
\begin{enumerate}
\item {\em Waypoint tracking (WT)\/}: Each robot is assigned a sequence of waypoints in the plane and they traverse these waypoints. The robots do not employ any collision avoidance and do not exchange messages. This simple building block is used in several other applications. The two global predicates of interest are $\mathit{Separation}$ and $\mathit{Collinear}$. A set of robots satisfy $\mathit{Separation}(d)$ at a given time if the minimum distance between all pairs is at least $d$. They satisfy $\mathit{Collinear}(\epsilon)$ if there exists a straight line passing within $\epsilon$ distance of their positions.

\item {\em Geocasting (GC)\/}: Each robot follows a sequence of waypoints as in WT and some of the robots geocast a message $m$ to a circular area $C$ in the plane. The key property of interest is that a robot receives this message iff it is located within $C$ during the time interval $[t+a, t+b]$, where $t$ is the time at which the message was sent. We call this property $Georeceive(a,b,C)$.

\item {\em Distributed Traffic Control (DTC)\/}. Each robot has to traverse a specified sequence of segments as in WT, however, when two robots attempt to traverse intersecting segments simultaneously (representing traffic intersections), then one of them has to acquire a lock on that intersection. The robot succeeding in obtaining the lock traverses its segment, while the others wait. Each intersection lock is managed by the robots executing a distributed mutual exclusion algorithm. The important properties here are separation and deadlock freedom.

\end{enumerate}

\taylor{Call ``harness functions'' something else, this is not a standard term as far as I'm aware}
One important component of \starl is the {\em trace writer\/} that is called by functions and applications to record observations. Observations after each message send and receive are recorded by default. The frequency of other observations and the amount of state information that is recorded at each observation are controlled by the observation recording functions.
In our experiments, we use two types of traces. First, for systems with four or fewer agents, the traces are recorded from the same number of Android devices executing application code. In these experiments, the position of each agent (wherever applicable) is obtained from a vision-based indoor positioning system.
%
Secondly, for generating traces for systems with dozens of agents we have created a {\em \starl discrete event simulator\/} that can execute many instances of a \starl application. Specifically, the simulator executes the actual \starl application code combined with harness functions that substitute Android's hardware specific functions and physical sensors, such as the WiFi interface, the local clock, and the location sensors. For example, to generate traces for $20$ robots, each robot is simulated on a PC by a process (with several threads).  Each process obtains the location of the simulated robot from a harness function that mimics the motion of the actual robot (in our case, the iRobot Create) in the simulated environment. Simulated robots can turn in place, move in straight lines, and travel in circular arcs. In a similar fashion, other harness functions provide the agent process access to simulated communication channels over which messages can be delayed and dropped. 
%
% Ground truth.
For this paper, we also record the ``true execution'' that generates each trace. For the traces from the deployed system, the true execution is obtained from a log of the actual positions and states of all the robots that is updated at a high sampling rate (higher than the observation frequency) as is maintained in a central PC with an accurate real-time clock. For the simulation traces, the simulator itself records snapshots of the entire system as a record of the true execution.


\taylor{reread next: trying to address real-time java concerns}
%
Since \starl is written in Java for Android, real-time issues related to memory management and garbage collection are a potential issue.
%
However, recall that for the soundness of our analysis (\ref{lem:soundi}), the only real-time requirement (from~\ref{def:sync}) is the following.
%
If an observation $\vv_i[j].\clk$ appears in the trace $\beta$ with sync accuracy $\sigma > 0$, then the state $\vv_i$ must have been visited within the real time interval $[ts-\sigma, ts+\sigma]$.
%
Here $ts$ is the timestamp derived from the (possibly inaccurate) local clock $\clk_i$ and $\sigma$ is the synchronization accuracy.
%
Similar assumptions are made for trace observations about messages sent and received.


When a {\em trace writer\/} instruction is executed in the Java program it first (1) creates the $\vv_i[j]$ entry in memory (based on the current values of the program variables and local clock) and then (2) issues an instruction to write this observation to the trace stored on disk.
%
Nondeterministic delays (such as the garbage collector starting, disk write delays, etc.) may indeed appear between steps (1) and (2), but these delays only affect when the $\vv_i[j]$ observation is written to the trace file, and does violate the above assumption (\ref{def:sync}).
















%At each point along this path, a small ammount of noise is added to the robot orientation and position to provide a more realistic simulation.
%Positions are periodically recalculated and sent to all simulated robots to mimic the physical implementation as best as possible. 
% Sayan: Not sure what you mean by best as possible.
%
 %in simulated system's environment. These harnesses duplicate the functionality of their Android counterparts by exchanging information with the simulation engine instead of physical hardware. Simulated executions behave identically to real executions and don't require applications to be rewritten for the different platform.
%\sayan{This second part is not that clear. Too many words that do not have clear meanings. Need another iteration.}


%
%Each entry in the trace file is accompanied by a timestamp from the phone's internal clock. Each execution of an application is stored in a separate trace file, and all files from an execution are marked with a unique execution ID to allow traces to be easily sorted.

%
%
%Using a vision system, the location and orientation of each robotic chassis is periodically calculated and broadcast over WiFi to the phones from a desktop computer. This serves as a pseudo-GPS location provider. All phones are connected to the same wireless network, be it ad-hoc or managed by a router, and exchange messages over UDP using a simple acknowledging protocol.

%% Real Traces


%% StarL Simulator: Simulator harness
%% Motion model and its justification
%
%To simulate a swarm of robots running StarL applications, a PC based simulator was constructed. This simulator is capable of executing all StarL code and any application using StarL. The core pieces of the framework which are specific to the Android platform, such as the Bluetooth and WiFi interfaces, are replaced with harness functions in simulated system executions. These harnesses duplicate the functionality of their Android counterparts by exchanging information with the simulation engine instead of physical hardware. Simulated executions behave identically to real executions and don't require applications to be rewritten for the different platform.


%% Specific applications


%The second application is an extension of the first with the following modification: 

%%% Chase

%The third application is a distributed race. All robots are provided with an ordered list of waypoints to travel to, but only one robot may visit each point. The first robot to arrive at each point informs the others that the point has been visited. Upon receiving this message, all robots remove that waypoint from their list and immediately begin travelling to the next unclaimed position. This repeats until all positions have been visited.
%



\subsection{Scalability}
\label{sec:scale}

The first set of experimental results serve to illustrate the scalability of the proposed approach.
We have collected a large number of traces from the three \starl applications, WT, GC, and LP, with $4$-$20$ participating agents.
The automaton model of the application is obtained from the Java code, and includes details of the physical motion model.
Since the robots have simple turn-and-move dynamics, their motion is modeled using simple rectangular differential inclusions (e.g., $a \leq \dot{x} \leq b$).
Our tool attempts to automatically check the relevant properties by first constructing appropriate formulas and then making the always or eventually queries to Z3. 
%1) Separation(d) - Ensures that any two robots in the system are always distance d apart. This distance is measured using L_{\infty}. 
%2) Line(epsilon) - Ensures that the robots 1,2,3 and 4 are within +/- epsilon distance from a line.
%3) geocast(a,b,C) - Ensures that for a circle C in the place, any message geocast to C at time t is received by and only by those robots that are in C at some time in the interval [t+a, t+b].
%
%

Table~\ref{tab:scale} shows the total time and memory usage for checking global properties for typical traces.
Owing to limited space, for each property we report the performance numbers for $4, 12$, and $20$ robots participating in the application.
The size of the formula used to verifying the global predicate (i.e., the formula for global predicate detection) is given in the last column.
In these traces, one observation is recorded roughly every $100$ milliseconds, so a trace of length $100$ approximately corresponds to $10$ seconds in real-time.
For all these traces with up to $20$ robots, the properties are checked within a couple of minutes, and in most cases within a few seconds!
These figures suggest that the approach can scale and in some cases may even be suitable for checking properties of distributed cyber-physical systems in real-time. 

For the {\em Separation\/} property, we check that all the participating robots {\em always\/} maintain a minimum separation of $d$ centimeters.
This requires a pair-wise comparison of distances.
Note that for the same trace with $12$ (and $20$) robots, $\mathit{Separation}(d = 2.5)$ holds, whereas $\mathit{Separation}(d = 10)$ does not.
We examined the true execution for these traces (the fine-grained simulation log), and observed that, indeed, for a duration of about $200 ms$ robots $6$ and $11$ came within $10$cm of each other.  

For the {\em Collinear \/} property, we check that all the robots {\em never \/} form a rough straight line (within $\epsilon$ distance of an ideal line).
This property is violated by the robots, which implies that there exists a time, when, in some execution corresponding to the recorded trace, all the robots form a rough line.
The Collinear property has more nonlinear terms than the Separation property and hence takes more time to verify (note, these traces have only $10$ observations).


For the {\em Georeceive\/} property, we check that for any time $t$ if a message $m$ is geocast at $t$, then a robot receives $m$ if and only it is located within a specified circle $C$ during the interval $[t, t+100 ms]$.
Hence robot $i$ will receive a message if and only if, for {\em some \/} $t' \in [t,t+100ms]$, the robot lies in $C$, and it does not receive the message if and only if, for the {\em entire \/} duration $[t,t+100ms]$, it is outside the region.
%
Checking whether the position of a robot is within the circle $C$ at a given time involves checking satisfiability of formulas involving real-valued polynomials.
In theory, this problem is decidable, but Z3 does not guarantee completeness.
For some of the traces, Z3 returns ``Unknown'' even when the predicate actually holds. 
%
%One can observe that the time taken to verify this property is linearly dependent upon the number of Geocast messages and the number of robots. This trend if observed in the experimental results where the time taken linearly increases with the number of robots. 
Checking {\em Georeceive \/} is much faster than Separation because it only involves checking the position of individual robots over short time intervals, as opposed to the distance between all pairs over the entire duration.  

The influence of sampling time (i.e. the time between two consecutive observations of a robot) over the total time taken for verification is shown 
in Table~\ref{tab:sampling}. The table reports the time taken to verify the $\mathit{Separation}(d = 10)$ property for distributed traces of real time 
$5$ minutes. The verification time with sampling period of 500 ms are always lesser than a minute for the traces of 5 mins even with 20 robots. This
suggests a promising approach for integrating this framework into run-time verification of distributed hybrid systems. It can be clearly observed from 
Table~\ref{tab:sampling} that verification time is inversely proportional to the sampling time. This is because, as the sampling time increases, the number 
of observation intervals decrease and hence the lower is the verification time.  Another key observation is that because of the soundness of the analysis,
the outputs with different sampling periods were always consistent. Hence, one could adaptively change the sampling time based on the application in order to 
improve the scalability of the approach with the benifits of sound analysis. 
% This suggests the approach that, in order to improve the scalability of the verification,
% one could adaptively change the sampling period and still gain the benifits of sound analysis.

%Also, another observation to be made is that verifying Geocast(a,b,C) is faster than verifying Separation(d) because, the complexity of the Geocast(a,b,C) predicate only increases linearly with the number of messages and hence increases linearly with respect to the number of robots. However, in order to verify Separation(d), we need to check that for any two robots, separation is maintained and hence it increases quadratically with the number of robots. The time taken by Line(epsilon) is more than Separation(d) and Geocast(a,b,C) because of the number of variables in the non-linear predicate.

  %whenever a message In the Geocast(a,b,C) column,  Also, in Line(10) column, we have verified that the robots 1,2,3 and 4 lie at a +/- 10 units distance from a line. From the table, it can be observed that for a system of 8 robots, in order to verifying that any two robots are always separated by 25 units distance takes 4.44 sec and a memory of 5.35 mb for a trace of size 100. In order to validate the results of verification, we do a very detailed simulation of the system (time step for simulation is the order of 1 ms) and check the predicate with respect to the detailed simulation.
%

%Also, in order to verify Geocast(a,b,C), 


	

\begin{table}[t]
\centering
% \begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Property  		&	Num. &	Trace  &	Result	&	Time	&	Memory	&	Formula	\\
			&	agents	&	len. &		&	(sec) 	&	(Mb)	&	Size (Kb)\\
\hline 
{\em Always\/}  	&	4	&	100	&	Yes	&	1.6	&	3.07	&	3.9	\\
$\mathit{Separation}$	&	12	&	100	&	Yes	&	14.1	&	8.66	&	14.9	\\
$(d= 25)$		&	20	&	100	&	Yes	&	81.1	&	18.6	&	31.6	\\
\hline
{\em Always\/}		&	4	&	100	&	Yes	&	1.6	&	3.07	&	3.9	\\
$\mathit{Separation}$	&	12	&	100	&	No	&	14.1	&	8.66	&	14.9	\\
$(d=10)$		&	20	&	100	&	No	&	81.1	&	18.6	&	31.6	\\
\hline
{\em Always Not\/} 	&	4	&	10	&	No	&	4.66	&	5.83	&	3.7	\\
$\mathit{Collinear}$	&	12	&	10 	&	No	&	12.21	&	12.91	&	10.9	\\
$(\epsilon = 100)$	&	20	&	10	&	No	&	25.68	&	25.66	&	18.4	\\
\hline
{\em Always\/}		&	4	&	100	&Yes	&	1.28	&	1.24	&	3.2	\\
$\mathit{Georeceive}$ 	&	12	&	100	&Yes	&	1.77	&	3.67	&	9.5	\\
			&	20	&	100	&Yes	&	1.91	&	8.35	&	16	\\
\hline
\end{tabular}
%  \end{center}
\vspace{5pt}
\caption{\small Running time and memory requirements of distributed trace analysis.} 
\label{tab:scale}
\end{table} 

\begin{table}[t]
\centering
% \begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|c|}
\hline
	Num.    &Sampling Time	&Sampling Time	&Sampling Time	&Sampling Time	\\
	agents	&  75 ms. 	&	150 ms.	&	250 ms. &	500 ms.	\\
\hline 
	8	&	TBF	&	TBF	&	22.07	&	9.58	\\
	12	&	TBF	&	TBF	&	34.16	&	16.43	\\
	16	&	TBF	&	TBF	&	49.36	&	24.18	\\
	20	&	TBF	&	TBF	&	67.82	&	34.94	\\
\hline

\end{tabular}
%  \end{center}
\vspace{5pt}
\caption{\small Running time (in seconds) for verification of separation property for different sampling periods.} 
\label{tab:sampling}
\end{table} 

\subsection{Precision of Analysis}
\label{sec:precision}

The precision of our analysis algorithm depends both on the precision of the static analysis (i.e., $\Pre{}{}{}$ and $\Post{}{}{}$ computations) and the accuracy of the dynamic information, namely the observation intervals inferred from the trace and bounds on variation of velocity.
In this section, we discuss how different levels of precision about the static and the dynamic analysis can result in different answers.
We consider traces for WT and the GC with $4$ robots.  
%
The table consists of three parts. The first part shows the outcome of the analysis for $\mathit{Separation}$ with $d=10 cm$.
When the uncertainty in the dynamically computed observation interval (OI) increases from local clock $\pm 10 ms$ to $\pm 20 ms$, Separation gets violated.
With increased uncertainty in the dynamically calculated values of the observation intervals, we get a more conservative overapproximation of the set of executions which violates Separation. Analogously, when the velocity bound (VB) increases from $\pm 20$ to $\pm 50 cm/s$, for the same observation interval, the property gets violated.
Of course, whether there exists a real execution that violates the property depends on the tightness of the observation interval and the velocity bounds.  

The second part of Table~\ref{tab:precision} shows the outcome of analysis for $\mathit{Georeceive}$ with varying the minimum message delays (i.e. $a$) from $0 ms$ to $50 ms$ in $\mathit{Georeceive(a, 100 ms, C)}$ while keeping the observation intervals constant at $\pm 5 ms$.
The final part of the table varies the observation interval from $\pm 5 ms$ to $\pm 20 ms$ while keeping the minimum message delay fixed at $0$.
The key observation here is that increasing either the static (model) or the dynamical (execution) uncertainties gives more conservative overapproximations.
% behaviors of the system and potentially varying one might induce more number of behaviors than varying another.
%The table consists of two main parts, First is verifying the Separation(d) predicate and second is the Geocast(a,b,C) predicate. The entities to be changed are the clock skews, velocities, and the message delays.

%and 

\begin{table}[t]
\centering
% \begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|}
\hline
Separation 	& VB $=\pm 0 cm/s$ 	& VB $=\pm 20 cm/s$	& VB $=\pm 50 cm/s$  \\
\hline 
OI $=\pm 5 ms$	& yes			&	yes 		& 	no 		\\
\hline
OI $=\pm 10 ms$	& yes			&	no 		& 	no 		\\
\hline
OI $=\pm 20 ms$	& no			&	no 		& 	no 		\\
\hline
\hline
Georeceive 	& VB $=\pm 0 cm/s$ 	& VB $=\pm 20 cm/s$	& VB $=\pm 50 cm/s$  \\
\hline 
delay $= 0 ms$	& yes			&	yes 		& 	yes 		\\
\hline
delay $= 20 ms$	& yes			&	yes 		& 	no 		\\
\hline
delay $= 50 ms$	& no			&	no 		& 	no 		\\
\hline
\hline
Georeceive 	& VB $=\pm 0 cm/s$ 	& VB $=\pm 20 cm/s$	& VB $=\pm 50 cm/s$  \\
\hline 
OI $=\pm 5 ms$	& yes			&	yes 		& 	yes 		\\
\hline
OI $=\pm 10 ms$	& yes			&	yes 		& 	no 		\\
\hline
OI $=\pm 20 ms$	& yes			&	no 		& 	no 		\\
\hline


\end{tabular}
%  \end{center}
\vspace{5pt}
\caption{\small The same trace with different levels of precision in static and dynamic analyses yield different conclusions.} 
\label{tab:precision}
\end{table} 
   

%  In the Separation(d) predicate, changing the clock skews increases the number of possible executions of the system and hence upon increasing clock skew, we get a counterexample execution of the system that violates the property. The same is case with increasing the velocity. However, both these are dependent and whether the property will hold or not for a given value of skew and velocity uncertainty is given in the table.
% 
%   In the Geocasting(a,b,C). I am increasing the vaue of a, i.e. delay and check whether the predicate will be satisfied for a different values of delay, skew and velocity uncertainty. It turns out that a small change in the value of delay will effect the predicate satisfaction than the clock skews.
% 
%   Please go through the table and let me know if you have any questions.


\subsection{Experience with Deadlock Detection}
As described earlier, the LP application traverses segments as in WT, however when two robots attempt to traverse intersecting segments simultaneously, then one of them acquires a lock on the intersection.
It is not hard to imagine that a deadlock might occur when a cycle is formed with each robot holding the lock on one intersection and waiting for the lock on the next.
%Also, a collision or a faulty robot may create a deadlock where other robots wait to get the lock back from the halted robot. 
We used our procedure to check for the global predicate {\em always (no-deadlock) \/}.
If the property is violated, then there is a potential execution that deadlocks\footnote{The feasibility of this execution will depend on whether the analysis is complete in this case.}.

Our tool was able to automatically detect distributed deadlocks in two traces with $4$ robots.
In the first trace, the algorithm detected that the property is violated because robot $1$ had obtained the token on all the intersections and it had halted because of its proximity to robot $2$. Then, since all the tokens were taken by robot $1$, all the other robots (i.e., robots $2$, $3$, and $4$) were all waiting for robot $1$.
Examination of the true execution revealed that this was indeed the case. 
%
In a second trace, the tool detected a deadlock between robots $3$ and $4$.
In this case, robot $3$ had finished its traversal of waypoints and robot $4$ could not reach its intended intersection waypoint because it was occupied by $3$. %However, no other bots were waiting for any token from bot 4 and each of the robots completed traversing their sequence of way points. 
These automatically discovered counterexamples illustrate that the procedure can be useful for finding corner cases that are commonly missed by programmers.
%However because the bot 4 could not proceed further, the algorithm detected it as a deadlock.

%An interesting observation is that detecting deadlocks would be reduced to checking dependency cycle detection if the {\em exact \/} information about {\em all the events\/} is known. However, in practice, this is seldom the case. Our algorithm detects the possiblility of a deadlock with the clock skews and message delays and further, it checks the possibility of deadlock in a conservative overapproximation of all the execution sequences of the system.
%
%\subsection{Pragmatics}
%\label{sec:useindeadlock}


% Basic Correctness

%%% Safe

%%% Unsafety

% Situations where we cannot detect predicates

%%% Too much clock skew

%%% Recordings are too infrequent

% Scalability 

%%% with size of automata state

%%% with size of traces

%% ???
